Database as a Service - Current Issues and Its Future

With the prevalence of applications in cloud, Database as a Service (DBaaS) becomes a promising method to provide cloud applications with reliable and flexible data storage services. It provides a number of interesting features to cloud developers, however, it suffers a few drawbacks: long learning curve and development cycle, lacking of in-depth support for NoSQL, lacking of flexible configuration for security and privacy, and high cost models. In this paper, we investigate these issues among current DBaaS providers and propose a novel Trinity Model that can significantly reduce the learning curves, improve the security and privacy, and accelerate database design and development. We further elaborate our ongoing and future work on developing large real-world SaaS projects using this new DBaaS model.

==> acknowledgements.tex <==
acknowledge Nuco Solutions for the industrial fundings

==> interview.tex <==
we summarize our interview results here.  Not too many, around 10 questions in depth shall be enough.

Which shall in line with our proposed solutions and our identified challenges in developing cloud applications using DaaS.

==> methodology.tex <==
explain how we conduct literrature review, what protocol we used, how we conduct the data analysis.
Same applied to on-line surveys and interviews.

Please check two sample papers I have pinned on the right panel in the general channel.

